Improving Neural Machine Translation with Pre-trained Representation

Monolingual data has been demonstrated to be helpful in improving the translation quality of neural machine translation (NMT). The current methods stay at the usage of word-level knowledge, such as generating synthetic parallel data or extracting information from word embedding. In contrast, the power of sentence-level contextual knowledge which is more complex and diverse, playing an important role in natural language generation, has not been fully exploited. In this paper, we propose a novel structure which could leverage monolingual data to acquire sentence-level contextual representations. Then, we design a framework for integrating both source and target sentence-level representations into NMT model to improve the translation quality. Experimental results on Chinese-English, German-English machine translation tasks show that our proposed model achieves improvement over strong Transformer baselines, while experiments on English-Turkish further demonstrate the effectiveness of our approach in the low-resource scenario.

==> abstract.tex <==
Monolingual data has been demonstrated to be helpful in improving the translation quality of neural machine translation (NMT).
The current methods stay at the usage of word-level knowledge, such as generating synthetic parallel data or extracting information from word embedding. In contrast, the power of sentence-level knowledge which is more complex and diverse, playing an important role in natural language generation, has not been fully exploited.
In this paper, we propose a novel structure which could leverage monolingual data to generate sentence-level representations. 
Then, we design a framework for integrating both source and target sentence-level representations into NMT model to improve the translation quality.
Experimental results on Chinese-English, German-English machine translation tasks show that our proposed model achieves improvement over strong Transformer baselines, while experiments on English-Turkish further demonstrate the effectiveness of our approach in the low-resource scenario. 


%Monolingual data has been demonstrated to be helpful in improving the translation quality of neural machine translation (NMT) systems, especially for the cases where high-quality parallel training data is not rich enough. In this paper, focusing on the Transformer, we propose a novel solution to better leverage monolingual data by utilizing the pre-trained deep representations. Our solution uses a bi-directional self-attention language model (BSLM) to obtain deep linguistic representations. We introduce approaches to integrate these pre-trained vectors into the Transformer: a weighted-fusion mechanism is used on the source side,  and a multi-task learning paradigm is employed on the target side. Experimental results on Chinese-English, German-English machine translation tasks show that our proposed model achieves improvement on standard data-sets, while experiments on English-Turkish further demonstrate the effectiveness of our method in the low-resource scenario.

==> intro.tex <==
Neural machine translation (NMT) based on an encoder-decoder framework~\cite{sutskever2014sequence,Cho2014Learning,Bahdanau2015Neural,Luong2015Effective} has obtained state-of-the-art performances on many language pairs~\cite{deng2018alibaba}.
Various advanced neural architectures have been explored for NMT under this framework, such as recurrent neural network (RNN)~\cite[RNNSearch]{Bahdanau2015Neural,Luong2015Effective}, convolutional neural network (CNN)~\cite[Conv-S2S]{gehring2016convolutional}, self-attention network~\cite[Transformer]{vaswani2017attention}.

Currently, most NMT systems only utilize the sentence-aligned parallel corpus for model training.
Monolingual data, which is larger and easier to collect, is not fully utilized limiting the capacity of the model.
Recently, several successful attempts have been made to improve NMT by incorporating monolingual data~\cite{gulcehre2015using,sennrich2016improving,Zhang2016Exploiting,poncelas2018investigating}, and reported promising improvements by utilizing linguistic information from monolingual data for NMT.  

However, these studies only focus on the usage of word-level information, e.g. extracting information from word embedding. Meanwhile, several methods such as ELMo \cite{peters2018deep}, GPT \cite{radford2018improving} and BERT \cite{devlin2018bert} have gained tremendous success by modeling sentence representation. So, the upcoming question is that whether the methods of acquiring and integrating sentence representations from them could be applied directly to machine translation or other natural language generation tasks. 


In this paper, we compare these methods and demonstrate it is non-trivial to propose new methods to acquire sentence representation and integrate it into NMT for three main reasons:
First, due to the limited amount of parallel data, the NMT network may not generate appropriate sentence representation, which is important in text generation. The pre-trained sentence representation could be an excellent complement to provide proper information for NMT.
Second, the current methods of acquiring pre-trained representations don't fully model the sequential information in the sentence, which is fundamental factor for getting a complete sentence-level representation.
Last, machine translation, which is a language generation task, has not been well studied. For example, in NMT the target translation is generated on the fly during the inference stage, most current methods could not benefit the decoder with the partially generated inputs.


To address the challenges above, we propose a solution to better leverage the pre-trained sentence representation to improve NMT as follows:
First, we propose a \textit{bi-directional self-attention language model} (BSLM) to acquire sentence representation which is trained by the monolingual data. 
The BSLM could capture the forward and backward sequential information from a sentence.


Then, we design an framework to integrate effectively task-specific information from pre-trained representation on both source and target sides. We propose a weighted-fusion mechanism for fusing the task-specific representation into the encoder. For the decoder, we use a knowledge transfer method to learn task-specific knowledge from the pre-trained representation.
This framework could be applied to various neural structures based on the encoder-decoder framework~\cite{Bahdanau2015Neural,gehring2016convolutional,vaswani2017attention} and language generation tasks.


To demonstrate the effectiveness of our approach, we implement it on the current state-of-the-art Transformer network~\cite{vaswani2017attention}.
Experimental results on Chinese-English and German-English translation tasks show that our approach improves over the Transformer baseline on the standard data-sets. 
Moreover, we show that on low resource language pair like English-Turkish, our approach leads to more improvements. 





==> model.tex <==
\begin{figure*}[ht]
    \centering
    \subfloat[Overview of the weighted-fusion mechanism used in the source side of Transformer.]{
     \label{fig:src side}
    \includegraphics[scale=.45]{source_side.pdf}}
    \subfloat[Overview of the weighted-fusion mechanism used in the source side of Transformer.]{
     \label{fig:trg side}
    \includegraphics[scale=.45]{target_side.pdf}}
    \label{fig:model}
    \caption{Overview of the weighted-fusion mechanism used in the source side of Transformer.}
    \end{figure*}

==> result_source_side.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l||c|c}
\hline
\textbf{Model} &\textbf{BLEU}&$\Delta$ \\
\hline
Transformer &44.59&$-$ \\
\hline
\ \ + Weighted-fusion (\it{first}) & 44.88& +0.29 \\
\ \ + Weighted-fusion (\it{deep}) & 45.34& \textbf{+0.75}  \\
\hline
\ \ + Knowledge Transfer (\it{first}) & 44.92 & +0.33   \\
\ \ + Knowledge Transfer (\it{deep})  & 45.06 & +0.47  \\
\hline
\end{tabular}
\caption{The comparison of translation qualities for our proposed methods used in the source side of the Transformer.}
\label{tab:result_source_side}
\end{table}


==> result_target_side.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l||c|c}
\hline
\textbf{Model} &\textbf{BLEU}&$\Delta$ \\
\hline
Transformer &44.59&$-$ \\
\hline
\ \ + Weighted-fusion (\it{first}) & 44.66& +0.07 \\
\ \ + Weighted-fusion (\it{deep}) & 43.93& -0.66  \\
\hline
\ \ + Knowledge Transfer (\it{first}) & 45.34 & +0.75   \\
\ \ + Knowledge Transfer (\it{deep})  & 45.45 & \textbf{+0.85}  \\
\hline
\end{tabular}
\caption{The comparison of translation qualities for our proposed methods used in the target side of the Transformer.}
\label{tab:result_target_side}
\end{table}

==> src_side.tex <==
\begin{figure}
\centering
\includegraphics[scale = 0.45]{figure/source_side.pdf}
\caption{Overview of the weighted-fusion mechanism used in the encoder of the Transformer.}
\label{fig: src}
\end{figure}

==> tr-en_r.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{l||cc|c}
\hline
\textbf{Model} &\textbf{NSD16}&\textbf{NST16} &$\Delta$ \\
\hline
Transformer &17.35	&13.42  &$-$ \\
\hline
\ \ + Our Approach &\textbf{18.61} &\textbf{14.35}&\textbf{+0.74} \\
\hline
\end{tabular}
\caption{Translation qualities on the TR$\rightarrow$EN experiments.}
\label{tab:tr-en_r}
\end{table}


==> trg_side.tex <==
\begin{figure}
\centering
\includegraphics[scale = 0.45]{figure/target_side.pdf}
\caption{Overview of the multi-task learning paradigm employed in the decoder of the Transformer.}
\label{fig: trg}
\end{figure}
